Frozen Transformers in Language Models Are Effective Visual Encoder Layers

This paper reveals that large language models (LLMs), despite being trained solely on textual data, are surprisingly strong encoders for purely visual tasks in the absence of language. Even more intriguingly, this can be achieved by a simple yet previously overlooked strategy -- employing a frozen transformer block from pre-trained LLMs as a constituent encoder layer to directly process visual tokens. Our work pushes the boundaries of leveraging LLMs for computer vision tasks, significantly departing from conventional practices that typically necessitate a multi-modal vision-language setup with associated language prompts, inputs, or outputs. We demonstrate that our approach consistently enhances performance across a diverse range of tasks, encompassing pure 2D and 3D visual recognition tasks (e.g., image and point cloud classification), temporal modeling tasks (e.g., action recognition), non-semantic tasks (e.g., motion forecasting), and multi-modal tasks (e.g., 2D/3D visual question answering and image-text retrieval). Such improvements are a general phenomenon, applicable to various types of LLMs (e.g., LLaMA and OPT) and different LLM transformer blocks. We additionally propose the information filtering hypothesis to explain the effectiveness of pre-trained LLMs in visual encoding -- the pre-trained LLM transformer blocks discern informative visual tokens and further amplify their effect. This hypothesis is empirically supported by the observation that the feature activation, after training with LLM transformer blocks, exhibits a stronger focus on relevant regions. We hope that our work inspires new perspectives on utilizing LLMs and deepening our understanding of their underlying mechanisms. Code is available at https://github.com/ziqipang/LM4VisualEncoding.

==> sections/1-introduction.tex <==
\vspace{-2mm}
\section{Introduction \textcolor{blue}{[Finished]}}
\vspace{-2mm}

The capabilities of large language models (LLMs) in generalization to various tasks have revolutionized the design of vision-language models (VLMs). Besides processing language tokens, LLMs illustrate the ability to interact with visual tokens and \emph{decode} them into tokenized output, exemplified by either projecting visual tokens to LLMs via linear layers~\citep{koh2023grounding, lin2023towards, merullo2022linearly, schwettmann2023multimodal} or cross-attention between visual and language tokens~\citep{alayrac2022flamingo, li2022blip, li2023blip, wang2023visionllm}. However, the discovery of processing visual information LLMs is surprising since they are trained entirely with texts and have never encountered visual input.

We push the direction of using LLMs for visual input to its limits with a straightforward yet overlooked approach: incorporating a \emph{frozen} transformer block in a \emph{pretrained} LLM as a general-purpose visual \emph{encoder} layer, directly processing the visual tokens. Concretely, our design is illustrated in Fig.~\ref{fig:architecture_teaser} and Fig.~\ref{fig:code_teaser}: (1) extract a \emph{frozen} LLM transformer block and append it behind the original visual encoder, (2) insert \emph{trainable} linear layers before and after the added LLM block to align the feature dimensions, (3) \emph{freeze} the LLM transformer but optimize the other modules as usual during training. Surprisingly, this simple design improves the performance across a wide range of tasks, including pure 2D and 3D recognition (image and point cloud classification), video understanding (action recognition), non-semantic tasks (motion forecasting), and multi-modal tasks (2D/3D visual question answering and image-text retrieval). Such enhancements are also general across multiple LLMs (LLaMA~\citep{touvron2023llama} and OPT~\citep{zhang2022opt}) and diverse transformer blocks.

\begin{figure}
    \centering
    \begin{subfigure}[tb]{0.60\linewidth}
    \vspace{-2mm}
    \caption{Architecture}
    \label{fig:architecture_teaser}
    \includegraphics[width=1.0\linewidth]{figures/architecture.pdf}
    \end{subfigure}
    \begin{subfigure}[tb]{0.39\linewidth}
    \caption{Pseudo Code}
    \label{fig:code_teaser}
    \includegraphics[width=1.0\linewidth]{figures/code.pdf}
    \end{subfigure}
    \vspace{-3mm}
    \caption{Our straightforward method of using a \emph{frozen} transformer block from \emph{pretrained} LLMs as a visual encoder layer. Visualized with an example of ViT~\citep{dosovitskiy2020image}. \textbf{(a)} Our design simply appends a frozen transformer block (pink) behind the regular visual encoder (gray). Only two trainable linear layers (green) are added to align the feature dimensions. \textbf{(b)} Pytorch-style pseudo code shows the simplicity of our approach.}
    \vspace{-6mm}
    \label{fig:teaser}
\end{figure}

Our discovery of using a pretrained LLM transformer block as a visual encoder layer is intriguing because it notably deviates from the conventional designs of vision-language models (VLMs). Our treating LLM transformers as \emph{encoders} (1) is independent of language prompts, inputs, or outputs; (2) can be trained from scratch without relying on pretrained backbones like CLIP~\citep{radford2021learning}; and (3) separate and simplify the usage of LLM into separate transformer blocks.

To comprehend the effectiveness of LLM transformer blocks in visual encoding, we propose the  \emph{information filtering} hypothesis: the pretrained transformer blocks distinguish informative visual tokens and augment their contribution to the latent representation. This hypothesis stems from our observation on multiple tasks that the feature activation illustrates better concentration on the informative regions after incorporating the frozen LLM transformer blocks.

In conclusion, we have made the following contributions and structured the paper accordingly:
\begin{itemize}[leftmargin=*, noitemsep, nolistsep]
    \item We discover that \emph{using a frozen transformer block from pretrained LLMs as a visual encoder layer} effectively enhances various tasks, which is straightforward yet overlooked.
    \item The benefits of frozen LLM transformers in visual encoding are general phenomena observed in varied LLMs and transformer blocks.
    \item We propose the \emph{information filtering hypothesis} to explain the effectiveness of frozen LLM transformers in processing visual tokens: the incorporated LLM blocks distinguish the informative tokens and amplify their effects.
\end{itemize}
We hope our fair comparison on diverse baselines, though not necessarily at full scale or achieving state-of-the-art, will bring attention to the intriguing application of using LLM transformer blocks as visual encoders and inspire new perspectives on understanding VLMs/LLMs.

==> sections/5-hypothesis-long.tex <==
\vspace{-2mm}
\section{Information Filtering Hypothesis}
\vspace{-2mm}
\label{sec:hypothesis}

This section explains how pretrained LLM transformers benefit visual tasks. In plain language, our hypothesis can be stated as below:

\mypar{Information filtering hypothesis.} The pretrained LLM transformer functions as a ``filter'' that \emph{distinguishes the informative tokens} and \emph{augments their contribution for the prediction} reflected in the feature activation, such as larger magnitudes or frequencies. 

In this section, we first describe and derive the hypothesis in detail with examples from image classification (Sec.~\ref{sec:hypothesis_story}). Then a series of quantitative evidence back up our qualitative observations in derivation (Sec.~\ref{sec:quantitative_evidence}). Finally, we discuss the applicability of our hypothesis to other tasks (Sec.~\ref{sec:hypothesis_other_tasks}).

\vspace{-2mm}
\subsection{Qualitative Derivation of Information Filtering Hypothesis \textcolor{blue}{[Finished]}}
\vspace{-2mm}
\label{sec:hypothesis_story}

\mypar{Sketch of derivation.} Our hypothesis origins from the intriguing feature activation pattern: the features better concentrate on the target objects after training with the LLM transformer (Fig.~\ref{fig:hypothesis}). However, the attention scores between the $\mathtt{CLS}$ token and visual tokens are still noisy and struggle at capturing foreground objects. More interestingly, the mechanism of $\mathtt{CLS}$ token indicates that the visual tokens output from the frozen LLM are not direct contributors to the final prediction. To explain the contradiction between the quality of features and attention scores, as well as bridge the gap between the final prediction and visual tokens, we finally arrive at the hypothesis that the frozen LLM transformers are implicitly selecting and augmenting the informative features.

\vspace{-2mm}
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/hypothesis.pdf}
    \vspace{-3mm}
    \caption{Visualization of feature activation for ViT and ViT-LLaMA, regarding both magnitudes and frequencies of features. We highlight that ViT-LLaMA demonstrates the emergent tendency of object segmentation compared to ViT, indicating the functionality of selecting informative tokens.}
    \vspace{-4mm}
    \label{fig:hypothesis}
\end{figure}

\mypar{Emergent concentration on informative tokens.} As stated in the ``sketch of derivation,'' our hypothesis originates from the emergent behavior that \emph{the feature activation highlights the informative tokens} after incorporating pretrained LLM transformers. In the analysis, we extract the activation of features after each inserted layer as Fig.~\ref{fig:hypothesis}, including the original ViT block $\mathbf{F}_E$, the attention layer $\mathbf{F}_{LM}^A$ and feedforward network $\mathbf{F}_{LM}^F$ in the LLM transformer $\mathbf{F}_{LM}$, and the second linear layer $\mathbf{F}_L^2$. Notably, we analyze the activation of features in terms of both \emph{magnitudes} (L2-norm after centering) and \emph{frequencies} (L2-norm of angles after Fourier transformation) as in Fig.~\ref{fig:hypothesis}.\footnote{Details of computation are in Sec.~\ref{sec:supp_visualization_details}.} Such a design is driven by the flexible formats that neural networks encode information, which include but are not limited to the scale and frequency of embeddings. The patterns in Fig.~\ref{fig:hypothesis} validate our design because different layers indeed show diverse preferences over magnitudes or frequencies.

After translating features into magnitudes or frequencies, we observe that token activation better captures the outlines of target objects after adding the LLM transformer, especially the magnitudes of $\mathbf{F}_L^2$ and frequencies of $\mathbf{F}_{LM}^A$ in Fig.~\ref{fig:hypothesis}. Their tendency to segment target objects is an emergent and surprising discovery in ViT-LLaMA because emergent segmentation only exists in self-supervised learned~\citep{caron2021emerging} or specially-designed~\citep{bohle2023b, shi2023top, yu2023white} ViTs. More importantly, the activation's concentration on the target objects is confusing to understand because ViT relies on the $\mathtt{CLS}$ token for prediction and the visual tokens beginning from the LLM layer $\mathbf{F}_{LM}^A$ are never directly supervised, \emph{i.e.}, their gradients are always zero. In fact, bridging these token features with the final prediction is the key to deriving our hypothesis. 

\begin{wrapfigure}{r}{0.40\textwidth}
  \begin{center}
    \includegraphics[width=0.40\textwidth]{figures/attention_scores.pdf}
  \end{center}
  \vspace{-3mm}
  \caption{Attention scores between the $\mathtt{CLS}$ token and visual tokens. The attention pattern from ViT is commonly noisy (left). Though ViT-LLaMA improves the concentration of target objects on a few heads, most of the attention heads are still noisy. Both good and bad attention heads from ViT-LLaMA are sampled for illustration purpose.}
  \vspace{-4mm}
  \label{fig:attention_scores}
\end{wrapfigure}

\mypar{Noisy attention weights.} In contrast to the feature activation, attention scores struggle to capture the relevant visual tokens for prediction. We investigate the attention scores between the $\mathtt{CLS}$ token and visual tokens in the last transformer block. For ViT and ViT-LLaMA, we are referring to the last self-attention block in $\mathbf{F}_E$ and the transformer of $\mathbf{F}_{LM}$, respectively. Ideally, attention scores that perfectly distinguish the target object should exhibit object segmentation patterns like DINO~\citep{caron2021emerging}. However, supervised ViT models commonly have noisy attention scores (left part in Fig.~\ref{fig:attention_scores}). Although ViT-LLaMA illustrates the ability of emergent segmentation in a few attention heads, most of the attention scores also suffer from attention scattering to unrelated regions. These observations contrast the patterns of feature activation and indicate that the benefits of LLM transformers cannot be simply attributed to better attention scores, since attention scores fail to reliably contribute correct visual tokens for the $\mathtt{CLS}$ token.

\mypar{Deriving the hypothesis.} Our previous visualization shows that feature activation concentrates on the target objects better than both the vanilla ViT activation and attention scores. This supports our informative filtering hypothesis that \emph{the inserted LLM transformers and linear layers distinguish the informative tokens}. Naturally, the downstream decoder $\mathbf{F}_D$ can predict with higher fidelity from these filtered token features. 

However, the above explanation is insufficient when the models are using the $\mathtt{CLS}$ token, \emph{e.g.} in image classification:  the visual token features beginning from $\mathbf{F}_{LM}^A$ are not direct input to the decoder and always receive zero gradients during training. The following derivation, which is the second half of our hypotheses, addresses this contradiction by proposing the critical role of \emph{augmenting informative tokens} with the added blocks.

Formally, we consider the self-attention inside $\mathbf{F}_{LM}^A$ and accordingly write the $\mathtt{CLS}$ token as,
\begin{equation}
\label{eqn:cls_attn_formula}
    z_{L}^2[\mathtt{CLS}] = \mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A \left( \sum_{v\in V} w_v \ z_{L}^1[v]\right),
\end{equation}
where $V$ is the set of visual tokens, $w_v$ is the attention scores between the $\mathtt{CLS}$ token and visual tokens $v$. The above Eqn.~\ref{eqn:cls_attn_formula} describes the process of (1) aggregating visual tokens $z_{L}^1[v]$ output from $\mathbf{F}_{L}^1$ guided by the attention scores $w_v$; (2) sequentially flowing through the MLP layers inside LLM transformer's attention head $\mathbf{F}_{LM}^A$, feedforward network $\mathbf{F}_{LM}^F$, and the second linear layer $\mathbf{F}_{L}^2$. Please note that this equation simplifies self-attention by removing the $\mathtt{CLS}$ token from input to focus on the effects of visual tokens.

Intuitively, we further separate the visual tokens into the subset of informative tokens $V_i$ and uninformative tokens $V_u$ and change Eqn.~\ref{eqn:cls_attn_formula} into,
\begin{equation}
    \label{eq:cls_informative_uninformative}
    z_{L}^2[\mathtt{CLS}] = \mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A \left( \sum_{i\in V_i} w_i \ z_{L}^1[i] + \sum_{u\in V_u} w_u \ z_{L}^1[u]\right).
\end{equation}

Using the same notation, the observation of our visualization can be stated as: the attention weights for informative tokens $\{w_i, i \in V_i\}$ are still noisy after incorporating the frozen LLM transformers, while the final visual tokens shown below have emergent concentration on the target regions.
\begin{equation}
    \label{eq:visual_token}
    z_{L}^2[i]=\mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A (z_{L}^1[i]),\ \text{where}\ i\in V_i
\end{equation}

Combining Eqn.~\ref{eq:cls_informative_uninformative} and Eqn.~\ref{eq:visual_token} inspires us to express our hypothesis on the connection between visual and $\mathtt{CLS}$ token as Eqn.~\ref{eq:hypothesis}, where the added modules $\mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A$ augment the informative tokens $V_i$ and lead to better prediction:
\begin{equation}
    \label{eq:hypothesis}
    z_{L}^2[\mathtt{CLS}] \quad \mathlarger{\propto}\quad 
    \sum_{i\in V_i} w_i 
    \underbrace{
    \left( \mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A (z_{L}^1[i]) \right)}_{z_{L}^2[i]} + 
    \sum_{u\in V_u} w_u 
    \underbrace{
    \left( \mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A (z_{L}^1[u]) \right)}_{z_{L}^2[u]}. \quad \text{[Hypothesis]}
\end{equation}
Eqn.~\ref{eq:hypothesis} holds equal under the special case of $\mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A$ being linear transformation. This equation explains how the informative tokens in Fig.~\ref{fig:hypothesis} are \emph{implicitly} reflected and supervised via the $\mathtt{CLS}$ token. It further clarifies that augmenting the informative tokens can benefit the final prediction though the attention scores $w_i$ are noisy, which completes our information filtering hypothesis for models with $\mathtt{CLS}$ tokens.

As a brief remark, our derivation builds upon three observed evidence: (1) visual tokens concentrating on informative parts; (2) noisy attention scores; (3) missing connection between the final visual tokens and the $\mathtt{CLS}$ token. Then our information filtering hypothesis builds a link between the visual tokens and the final output for the scenarios with or without a $\mathtt{CLS}$ token. 

\vspace{-2mm}
\subsection{Quantitative Evidence \textcolor{blue}{[Finished]}}
\vspace{-2mm}
\label{sec:quantitative_evidence}

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth]{figures/token_miou_concise.pdf}
    \vspace{-3mm}
    \caption{Pseudo masks generated from ViT-LLaMA's feature activation significantly outperform the masks from attention scores, which directly supports our hypothesis. In addition, the mask quality is also better for ViT-LLaMA ($\mathbf{F}_{L}^2$) than vanilla ViT, indicating the benefits of adding frozen language transformers. More discussion in Sec.~\ref{sec:quantitative_evidence}.}
    \vspace{-4mm}
    \label{fig:token_miou}
\end{figure}

The qualitative observation in the previous Sec.~\ref{sec:hypothesis} can be further supported with quantitative evidence. To quantitatively assess the fidelity of feature activation and attention scores, we first generate pseudo masks from them, then use the mIoU (mean intersection-over-union) between the pseudo and ground truth masks as the evaluation metric. Finally, the pseudo masks predicted from the features of ViT-LLaMA have larger mIoU compared to the attention scores and ViT features. Thus, it supports our \emph{information filtering} hypothesis that the inserted LLM-related modules distinguish and augment the informative token features.

\mypar{Ground truth masks.} We choose the ImageNet-S~\citep{gao2022luss} dataset because it provides segmentation annotation for the ImageNet images. Then the target regions on each image are intuitively defined as the union of masks with the same class label as the image. These are the ground truth for calculating the mIoU with the pseudo-masks from feature activation or attention scores. 

\mypar{Pseudo masks.} To generate pseudo masks from feature activation, we are motivated by Fig.~\ref{fig:hypothesis} and treat the highly-activated regions as the final pseudo-mask. To generate pseudo masks with attention scores, we first sum the scores from all the attention heads and follow a similar procedure of treating highly-scored regions as pseudo masks. Although the process is straightforward, we notice that selecting the thresholds for activation or score significantly affects the quality of pseudo masks. Therefore, we always automatically choose the threshold maximizing the mIoU between the pseudo and ground truth masks to avoid threshold tuning and enable a fair comparison. More details and specific algorithms are described in Sec.~\ref{sec:supp_quant_hypothesis_details}.

\mypar{Results and analysis.} We compare the quality of pseudo masks by their mIoU in Fig.~\ref{fig:token_miou}. For each type of feature, we only visualize the one with a larger mIoU from the activation of magnitude or frequency for clarity, and display the complete statistics in Sec.~\ref{sec:supp_miou_numbers}. As illustrated in Fig.~\ref{fig:token_miou}, both ViT-S-LLaMA and ViT-B-LLaMA have better pseudo mask quality from feature activation than attention scores. This directly supports our hypothesis that the features $\{\mathbf{F}_{L}^2 \cdot \mathbf{F}_{LM}^F \cdot \mathbf{F}_{LM}^A (z_{L}^1[i])|i\in V_i\}$ contribute more reliably than attention scores $\{w_i|i\in V_i\}$. We additionally notice that the pseudo masks from ViT-LLaMA generally have larger mIoU compared to ViT, which reflects the advantages of training ViTs with frozen language transformers. However, we would like to point out that the mIoU of pseudo masks is an intuitive but lossy metric to quantify feature representation because neural networks can encode information into other formats. Therefore, developing better measurements to compare individual network layers will be meaningful for future work.

\vspace{-2mm}
\subsection{Information Filtering Hypothesis on Diverse Tasks}
\label{sec:hypothesis_other_tasks}
\vspace{-2mm}

The previous sections mainly discuss our information filtering hypothesis on the task of image classification. Since frozen transformers are applicable for various tasks (Sec.~\ref{sec:application}), we provide additional observations on other tasks in this section.

\mypar{Action recognition.} We qualitatively analyze the activation patterns of action recognition by visualizing the feature activation of video tokens in Fig.~\ref{fig:video_activation}. Different from image tokens with shape $H\times W$, the visual tokens span both spatially and temporally in videos with shape $T\times H\times W$. Therefore, the token activation in Fig.~\ref{fig:video_activation} is considered jointly across all the frames instead of separately on each individual frame. Since VideoMAE~\citep{tong2022videomae} uses pooling instead of a $\mathtt{CLS}$ token for classification, the video tokens are directly supervised during the training time and exhibit relatively reasonable activation patterns, compared to image classification activation in Fig.~\ref{fig:hypothesis}. However, we notice that adding the LLaMA transformer better concentrates the video tokens to the hands and manipulated objects, as illustrated in the rows of ``low threshold.'' When raising the threshold to a higher value, we further observe that ViT-S-LLaMA has better ability in \emph{selecting video tokens temporally} -- the model accurately focuses on the middle frames with actual manipulation. Therefore, we conclude that the informative video tokens are indeed distinguished and augmented in action recognition, which aligns with the information filtering hypothesis.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/video_action_recognition.pdf}
    \vspace{-3mm}
    \caption{Visualization of video token activation. Different from images, the video tokens are jointly activated both spatially and temporally ($T\times H\times W$) instead of on each individual frame ($H\times W$). Every video token in this figure is a cube with shape $2\times 16\times 16$. After adding the LLM transformer, the model better \emph{concentrates on the target object and hands} (``low threshold'' lines) and more accurately \emph{focuses on frames with hand-object interaction} (``high threshold'' lines).}
    \vspace{-4mm}
    \label{fig:video_activation}
\end{figure}

\mypar{Point cloud recognition.}

\vspace{-2mm}
\subsection{Discussion \textcolor{blue}{[Finished]}}
\vspace{-2mm}
\mypar{Perspective of usable information.} We supplement the opinions from~\cite{xu2020theory} that greatly inspire our investigation of the information filtering hypothesis.~\cite{xu2020theory} proposes that a well-trained neural network layer can be considered as a \emph{decipher} adding usable information into the features and enabling subsequent modules to better infer the latent information. In our information filtering hypothesis, the incorporated modules are indeed acting as \emph{deciphers} that enlarge the contribution of usable tokens and benefit downstream predictions. 

\mypar{Limitations.} Though our information filtering hypothesis explains how the performance improves with frozen LLM transformers, we notice that several intriguing phenomena are not yet covered. First, the current hypothesis is unable to analyze the utilities of different layers separately. Second, the hypothesis does not explain how the training dynamics facilitate the visual token features to cooperate with the frozen language transformer.

==> tables/2d-vision-language.tex <==
\begin{table}[t]
\centering
\resizebox{0.70\textwidth}{!}{
\begin{tabular}{l|cccc|ccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{4}{c|}{VQAv2 (Tes-dev)} & \multicolumn{3}{c}{Flickr30k (Val)} \\
    & Overall & Yes/No & Number & Other & IR@1 & IR@5 & IR@10 \\
    \midrule
    METER & 69.60 & 85.08 & 47.82 & 61.37 & 49.66 & 80.86 & 89.48 \\
    + LLaMA & \textbf{70.23} & \textbf{85.70} & \textbf{48.98} & \textbf{61.89} & \textbf{50.22} & \textbf{82.26} & \textbf{90.08} \\
    \bottomrule
  \end{tabular}
}
\vspace{-2mm}
  \caption{Frozen LLaMA transformer improves 2D vision-language performance on the framework of METER~\cite{dou2022empirical}. We append the final LLaMA layer after the cross-modal fusion module in METER. The training setup on VQAv2 and Flickr30k follows~\cite{dou2022empirical, shi2023top}.}
  \vspace{-4mm}
  \label{tab:2dvl}
\end{table}

==> tables/imagenet-vit-old.tex <==
\begin{table}[t]
\centering
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{l|c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}}
    \toprule
    Model & ImageNet & ImageNet-C & ImageNet-A & ImageNet-SK & ImageNet-R \\
    \midrule
    ViT-T & 72.1 & 43.9 & 7.7 & 19.6 & 32.3 \\
    ViT-T-LLaMA & \textbf{73.2} & \textbf{45.8} & \textbf{8.7} & \textbf{20.6} & \textbf{33.8} \\
    \midrule
    ViT-S & 80.1 & 57.2 & 20.5 & 28.9 & 42.1 \\
    ViT-S-LLaMA & \textbf{80.7} & \textbf{58.7} & \textbf{22.7} & \textbf{30.5} & \textbf{42.8} \\
    \midrule
    ViT-B* & 78.9 & 58.1 & 21.6 & 29.3 & 40.5 \\
    ViT-B-LLaMA & \textbf{80.6} & \textbf{60.6} & \textbf{24.6} & \textbf{30.4} & \textbf{40.9}  \\
    \bottomrule
  \end{tabular}
}
\vspace{-3mm}
  \caption{Incorporating the single transformer block from LLaMA to ViT models consistently improves both accuracy (ImageNet) and robustness (ImageNet-$\{$C,A,SK,R$\}$). For ViT-T and ViT-S, we followed the training setup in DeiT~\citep{touvron2021training} and reproduced their accuracy. *Note that, while following the training setup for ViT-B in DeiT, we cannot reproduce the reported result in DeiT -- the similar reproduction issue has been noted, \emph{e.g.}, as in this \href{https://github.com/facebookresearch/deit/issues/195}{link}. Nonetheless, we ensured the same configuration for a fair comparison between our ViT-B and ViT-B-LLaMA. 
  % For ViT-T and ViT-S, we followed the training setup in DeiT~\citep{touvron2021training} and reproduced their accuracy. *Note that, due to the absence of the open-sourced training script for ViT-B in DeiT (check this \href{https://github.com/facebookresearch/deit/blob/main/README_deit.md\#training}{link}), we applied DeiT's configuration used for ViT-T and ViT-S to ViT-B, resulting in a lower performance than reported in DeiT (the similar reproduction issue has been noted as in this \href{https://github.com/facebookresearch/deit/issues/195}{link}). Nonetheless, we ensured the same configuration for a fair comparison between our ViT-B and ViT-B-LLaMA. 
  }
  \vspace{-6mm}
  \label{tab:imagenet-vit}
\end{table}
